Towards Counterfactual Fairness-aware Domain Generalization in Changing Environments

Recognizing the prevalence of domain shift as a common challenge in machine learning, various domain generalization (DG) techniques have been developed to enhance the performance of machine learning systems when dealing with out-of-distribution (OOD) data. Furthermore, in real-world scenarios, data distributions can gradually change across a sequence of sequential domains. While current methodologies primarily focus on improving model effectiveness within these new domains, they often overlook fairness issues throughout the learning process. In response, we introduce an innovative framework called Counterfactual Fairness-Aware Domain Generalization with Sequential Autoencoder (CDSAE). This approach effectively separates environmental information and sensitive attributes from the embedded representation of classification features. This concurrent separation not only greatly improves model generalization across diverse and unfamiliar domains but also effectively addresses challenges related to unfair classification. Our strategy is rooted in the principles of causal inference to tackle these dual issues. To examine the intricate relationship between semantic information, sensitive attributes, and environmental cues, we systematically categorize exogenous uncertainty factors into four latent variables: 1) semantic information influenced by sensitive attributes, 2) semantic information unaffected by sensitive attributes, 3) environmental cues influenced by sensitive attributes, and 4) environmental cues unaffected by sensitive attributes. By incorporating fairness regularization, we exclusively employ semantic information for classification purposes. Empirical validation on synthetic and real-world datasets substantiates the effectiveness of our approach, demonstrating improved accuracy levels while ensuring the preservation of fairness in the evolving landscape of continuous domains.

==> intro.tex <==
\begin{comment}
    Domain Generalization (DG)~\cite{zhou2022domain} pertains to the development of algorithms that empower a model to generalize its learned knowledge from a set of source domains to entirely new, unencountered domains. The aim is to enhance the model's robustness and effectiveness when confronted with domain shifts, thereby facilitating improved performance and reliability in real-world applications. 
\end{comment}
Data distribution may progressively evolve across a continuum of sequential domains in reality. Evolving domain generalization~\cite{wang2022evolving} involves constructing models capable of learning invariant representations across distinct periods or sequences, thereby extending the generalization capability to evolving data distributions over time. By bridging the temporal gap between source and target domains, this paradigm contributes to more adaptive and resilient machine learning solutions, particularly in scenarios characterized by dynamic environmental changes or evolving data streams. 

As an increasing array of methodologies extends domain generalization to encompass continuously evolving dynamic environments, there is a notable tendency to prioritize accuracy enhancement, often neglecting the equitable treatment of model performance across novel sequences of domains. However, fairness, which equally constitutes a significant concern within the domain of machine learning, is a facet that we must not disregard. A sensitive feature is defined as an attribute that contains protected information about individuals or groups within a dataset. This information may encompass characteristics such as race, gender, religion, or socioeconomic status, which are safeguarded by ethical considerations, legal regulations, or societal norms. For instance, a recent news article in The New York Times reported that during the COVID-19 pandemic, systemic algorithms exhibited an escalating level of discrimination against African American individuals in the context of bank loans~\cite{miller2020algorithm}. Causal models have been widely applied in machine learning to address issues related to model fairness. Structural Causal Models (SCMs)~\cite{2001Causality} provide a means of explaining machine learning model predictions. Analyzing causal graphs and paths helps understand how the model's predictions for different groups are formed, thereby identifying and addressing potential unfair factors. Simultaneously, to analyze fairness based on SCMs, a concept known as \textbf{counterfactual fairness} \cite{kusner2017counterfactual} has been introduced. This concept seeks to minimize the impact on predicted values when counterfactual interventions are applied to sensitive attributes. In the context of dynamically evolving environments, we propose a framework, denoted as \textbf{D}isentanglement for \textbf{C}ounterfactual \textbf{F}airness-aware \textbf{D}omain \textbf{G}eneralization (DCFDG), designed to address the issue of counterfactual fairness.

Our objective can be succinctly summarized as aiming to enhance the model's generalization capacity across unfamiliar domain sequences while concurrently ensuring counterfactual fairness in decision-making. Therefore, to model the relationships among sensitive attributes, environmental information, and semantic information, we partition the exogenous variables into four latent variables:  1) semantic information caused by sensitive attributes, 2) semantic information not caused by sensitive attributes, 3) environmental information caused by sensitive attributes, and 4) environmental information not caused by sensitive attributes. Among these, we posit that the distribution of semantic information remains invariant across all domains, whereas the distribution of environmental information varies with changes in the environment. Here, the data feature $X$ is composed of two components, wherein sensitive attribute $A$ directly causes a subset of features ($X_s$), while another subset of features ($X_{ns}$) is not directly influenced by $A$ but may still exhibit correlations with it. They are encoded in the latent space as the aforementioned first two exogenous variables. The advantages of this partitioning will be elucidated in the section detailing the causal structure of DCFDG. By employing such an approach, we skillfully disentangle environmental information and sensitive attributes from the embedded representation of classification features, ensuring a reduction in the impact of environmental changes on the model while concurrently upholding its decision fairness. In conclusion, our \textbf{contributions} can be summarized as follows:

1. We introduce a novel causal structure framework, DCFDG, which adeptly addresses data distributions that evolve within dynamic environments and are influenced by sensitive information. And we theoretically analyze the Evidence Lower Bound (ELBO) that should be considered within evolving environments.
    \begin{comment}
        \item Building upon the causal structure of DCFDG and incorporating the principles of variational inference, we theoretically analyze the Evidence Lower Bound (ELBO) that should be considered within evolving environments.
    \end{comment}
    
    2. Experimental results conducted on both synthetic and real-world datasets demonstrate that DCFDG exhibits superior predictive capabilities compared to existing exogenous variable disentanglement methods, while concurrently ensuring fairness.
    
    3. We introduce a novel synthetic dataset, $\mathbf{Fair-circle}$, specifically designed to address fairness issues in dynamically changing environments. This dataset presents a fresh perspective on constructing new datasets for this problem domain.

